Picasso: Memory-Efficient Graph Coloring Using Palettes With Applications in Quantum Computing

A coloring of a graph is an assignment of colors to vertices such that no two neighboring vertices have the same color. The need for memory-efficient coloring algorithms is motivated by their application in computing clique partitions of graphs arising in quantum computations where the objective is to map a large set of Pauli strings into a compact set of unitaries. We present Picasso, a randomized memory-efficient iterative parallel graph coloring algorithm with theoretical sublinear space guarantees under practical assumptions. The parameters of our algorithm provide a trade-off between coloring quality and resource consumption. To assist the user, we also propose a machine learning model to predict the coloring algorithm's parameters considering these trade-offs. We provide a sequential and a parallel implementation of the proposed algorithm. We perform an experimental evaluation on a 64-core AMD CPU equipped with 512 GB of memory and an Nvidia A100 GPU with 40GB of memory. For a small dataset where existing coloring algorithms can be executed within the 512 GB memory budget, we show up to 68x memory savings. On massive datasets we demonstrate that GPU-accelerated Picasso can process inputs with 49.5x more Pauli strings (vertex set in our graph) and 2,478x more edges than state-of-the-art parallel approaches.

==> IPDPS24/Floats/Table/mem-compare.tex <==
\begin{table}[!htp]\centering
\caption{Memory comparison (in GB)}\label{tab:mem-compare}
\scriptsize
\begin{tabular}{lrrrrrr}\toprule
Problem & &\multicolumn{2}{c}{Picasso} & & \\\cmidrule{1-1}\cmidrule{3-4}
&Colpack & & &Kokkos-EB &ECL-GC-R \\\midrule
H6\_3D\_sto3g &0.38 &\textbf{0.08} &0.23 &1.19 &0.30 \\
H6\_2D\_sto3g &1.52 &\textbf{0.16} &0.90 &4.50 &0.77 \\
H6\_1D\_sto3g &1.68 &\textbf{0.17} &0.97 &4.93 &0.83 \\
H4\_2D\_631g &2.72 &\textbf{0.20} &1.24 &6.81 &1.10 \\
H4\_3D\_631g &5.66 &\textbf{0.31} &3.10 &15.69 &2.37 \\
H4\_1D\_631g &10.77 &\textbf{0.38} &4.31 &23.69 &3.51 \\
H4\_2D\_6311g &140.23 &\textbf{2.06} &57.12 &NA &NA \\
\bottomrule
\end{tabular}
\end{table}

==> IPDPS24/Floats/Table/quality-compare.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{comment}
\begin{table*}[!htp]\centering
\caption{Quality and memory comparison with Sequential Greedy Color}\label{tab:quality-mem-cpu }
\scriptsize
\begin{tabular}{l|rrrrr|rr|rr}\toprule
Problem &\multicolumn{5}{c|}{Greedy Coloring (ColPack)}  &\multicolumn{2}{c|}{\pic ( $\calP = 12.5\%, \alpha = 2$)} &\multicolumn{2}{c}{\pic ( $\calP = 3\%, \alpha = 30$)} \\\cmidrule{2-6}\cmidrule{7-10}
&LF &SL &DLF &ID &Mem. (GB) &Avg. Cols. &Mem. (GB) &Avg. Cols &Mem. (GB) \\\midrule
H6\_3D\_sto3g &2479 &902 &901 &952 &0.38 &1425.4 &0.08 &\textbf{880.6} &0.23 \\
H6\_2D\_sto3g &5389 &1598 &\textbf{1580} &1634 &1.52 &2901.5 &0.16 &1587.4 &0.90 \\
H6\_1D\_sto3g &5771 &1672 &\textbf{1601} &1689 &1.68 &3036.1 &0.17 &1650.4 &0.97 \\
H4\_2D\_631g &10049 &1922 &\textbf{1694} &1917 &2.72 &3579.8 &0.20 &1784.2 &1.24 \\
H4\_3D\_631g &15883 &2729 &2633 &2668 &5.66 &5431.4 &0.31 &\textbf{2606} &3.10 \\
H4\_1D\_631g &19412 &3241 &\textbf{2943} &3233 &10.77 &6538 &0.38 &3212.8 &4.31 \\
H4\_2D\_6311g &72493 &8615 &\textbf{6944} &8628 &140.23 &22463.8 &2.06 & 8917.4 & 57.12 \\
\bottomrule
\end{tabular}
\end{table*}


%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Quality and memory comparison with Sequential Greedy Color}\label{tab:quality-mem}
\scriptsize
\begin{tabular}{lrrrrrrrrrrrrrr}\toprule
& & & & & &\multicolumn{3}{c}{Picasso} & & & & & \\\cmidrule{7-9}
Problem &\multicolumn{5}{c}{Greedy Coloring (ColPack)} &\multicolumn{2}{c}{} &\multicolumn{2}{c}{} &\multicolumn{2}{c}{Kokkos-EB} &\multicolumn{2}{c}{ECL-GC-Reduction} \\\cmidrule{1-14}
&LF &SL &DLF &ID &Mem. (GB) &Avg. Cols. &Mem. (GB) &Avg. Cols. &Mem. (GB) &Avg. Cols. &Memory &Col. &Mem. (GB) \\\midrule
H6\_3D\_sto3g &2479 &902 &901 &952 &0.38 &1425.4 &\textbf{0.08} &\textbf{880.6} &0.23 &1040.2 &1.19 &943 &0.30 \\
H6\_2D\_sto3g &5389 &1598 &\textbf{1580} &1634 &1.52 &2901.5 &\textbf{0.16} &1587.4 &0.90 &1749.2 &4.50 &1596 &0.77 \\
H6\_1D\_sto3g &5771 &1672 &\textbf{1601} &1689 &1.68 &3036.1 &\textbf{0.17} &1650.4 &0.97 &1815.8 &4.93 &1642 &0.83 \\
H4\_2D\_631g &10049 &1922 &\textbf{1694} &1917 &2.72 &3579.8 &\textbf{0.20} &1784.2 &1.24 &1772.7 &6.81 &1860 &1.10 \\
H4\_3D\_631g &15883 &2729 &2633 &2668 &5.66 &5431.4 &\textbf{0.31} &\textbf{2606.0} &3.10 &2478.5 &15.69 &2596 &2.37 \\
H4\_1D\_631g &19412 &3241 &\textbf{2943} &3233 &10.77 &6538.0 &\textbf{0.38} &3212.8 &4.31 &3426.2 &23.69 &3098 &3.51 \\
H4\_2D\_6311g &72493 &8615 &\textbf{6944} &8628 &140.23 &22463.8 &\textbf{2.06} &8917.4 &57.12 &NA &NA &NA &NA \\
\bottomrule
\end{tabular}
\end{table*}
\end{comment}

\begin{table}[!htp]\centering
\caption{Quality comparisons of the algorithms. Norm.:$\calP = 12.5\%, \alpha = 2$; Aggr.:$\calP=3\%, \alpha=30$}\label{tab:quality-compare}
\scriptsize
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|rrrr|rr|rr}\toprule
Problem &\multicolumn{4}{c|}{Greedy Coloring (ColPack)} &\multicolumn{2}{c|}{\pic{}} &Kokkos-EB &ECL-GC\\\cmidrule{1-9}
&LF &SL &DLF &ID & Norm.& Aggr.& & \\\midrule
H6\_3D\_sto3g &2479 &902 &901 &952 &1425.4 &\textbf{880.6} &1040.17 &943 \\
H6\_2D\_sto3g &5389 &1598 &\textbf{1580} &1634 &2901.5 &1587.4 &1749.17 &1596 \\
H6\_1D\_sto3g &5771 &1672 &\textbf{1601} &1689 &3036.1 &1650.4 &1815.83 &1642 \\
H4\_2D\_631g &10049 &1922 &\textbf{1694} &1917 &3579.8 &1784.2 &1772.67 &1860 \\
H4\_3D\_631g &15883 &2729 &2633 &2668 &5431.4 &\textbf{2606} &2478.50 &2596 \\
H4\_1D\_631g &19412 &3241 &\textbf{2943} &3233 &6538 &3212.8 &3426.17 &3098 \\
H4\_2D\_6311g &72493 &8615 &\textbf{6944} &8628 &22463.8 &8917.4 &NA &NA \\
\bottomrule
\end{tabular}
}
\end{table}
